Yetter-Drinfeld modules over Nichols systems and their reflections

We construct reflection functors for Yetter-Drinfeld modules over Nichols systems and discuss their fundamental properties. We will obtain properties about the geometry of the support of Nichols systems and their Yetter-Drinfeld modules, by looking at iterated reflections. We will also study the maximal subobject of Yetter-Drinfeld modules over Nichols systems and find a special morphism, that we name Shapovalov morphism, whose kernel coincides with this maximal subobject. Moreover, we will use this morphism to characterize properties about the reflections of the Yetter-Drinfeld modules. We calculate an explicit formula of the Shapovalov morphism in the case where the Nichols system is of group type. We will use the formula to calculate its kernel in the components of degree $2$ and to ascribe the theory of reflections of Yetter-Drinfeld modules over Nichols systems of diagonal type with the reflection theory of Dynkin diagrams. We will also apply and specify the theory to the Yetter-Drinfeld modules over Nichols systems that are obtained by inducing comodules of the Nichols systems, a construction that is reminiscent of Verma modules in the representation theory of Lie algebras. For Nichols systems of diagonal type we will obtain the result, that such an induced objects irreducibility can be characterized by a polynomial that is given by the positive roots of its Nichols system. This polynomial appeared in previous works and is known as Shapovalov determinant. Finally, we will apply the theory to some specific examples of Nichols algebras of nonabelian group type and to some examples of Nichols algebras of diagonal type.

==> sections/yd_modules_of_nichols_systems/resolutions.tex <==
% UNUSED

\section{Resolutions}

Let $\scr{N}$ be a pre-Nichols system and let $Q := \nsalg{\scr{N}}$ and $N_j := \scr{N}_j$ for all $j \in \mathbb{I}$. 
Let $\Gamma$ be an abelian group, such that $\ndZ^\theta \subset \Gamma$.

\begin{rema}
    Let $V \in \ydcat{Q}{\scr{C}}$ and $U$ be a $Q$-subcomodule of $V$. Recall that by \Cref{lem_action_is_yd_morphism} we have that $\act^Q_V : \ydind{Q}{U} \rightarrow V$ is a morphism in $\ydcat{Q}{\scr{C}}$.
\end{rema}

\begin{defi}
    Let $X,V \in \ydcat{Q}{\scr{C}}$ and $f: V \rightarrow X$ a morphism in $\ydcat{Q}{\scr{C}}$.
    Let $U$ be a $Q$-subcomodule of $V$, such that the sequence
    \begin{align*}
        \ydind{Q}{U} \xrightarrow{ \act^Q_V } V \xrightarrow{f} X
    \end{align*}
    is exact. Then $\ydind{Q}{U}$ is called a \textbf{resolution of $(V,f)$}.
    
    A \textbf{resolution of $V$} is a sequence $(V_0,V_1,\ldots)$ of objects in $\ydcat{Q}{\scr{C}}$, such that $V_0 = 0$, $V_1=V$, $V_2$ is a resolution of $(V,V\rightarrow 0)$ and for $i \ge 3$ $V_i$ is a resolution of $(V_{i-1},\act^Q_{V_{i-2}})$.
\end{defi}

\begin{exa}
    Let $V \in \ydcat{Q}{U}$ be homogeneously generated $\Gamma$-graded. We are interested in the resolution of $V$. Let $V_0=0$, $V_1 = V$.
    Then by \Cref{prop_action_induces_epimorphism_from_induced_module} we know that
    \begin{align*}
        \ydind{Q}{\gencomp{V}} \xrightarrow{\act^Q_V} V \rightarrow 0
    \end{align*}
    is exact. Hence let $V_2 = \ydind{Q}{\gencomp{V}}$. TODO
\end{exa}
